Adaptive Mesh Refinement for arbitrary initial Triangulations

We introduce a simple initialization of the Maubach bisection routine for adaptive mesh refinement which applies to any conforming initial triangulation and terminates in linear time with respect to the number of initial vertices. We show that Maubach's routine with this initialization generates meshes that preserve shape regularity and satisfy the closure estimate needed for optimal convergence of adaptive schemes. Our ansatz allows for the intrinsic use of existing implementations.

==> Pictures/kuhntucker.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bisection"
%%% End:

